Spaceprint: a Mobility-based Fingerprinting Scheme for Public Spaces

In this paper, we address the problem of how automated situation-awareness can be achieved by learning real-world situations from ubiquitously generated mobility data. Without semantic input about the time and space where situations take place, this turns out to be a fundamental challenging problem. Uncertainties also introduce technical challenges when data is generated in irregular time intervals, being mixed with noise, and errors. Purely relying on temporal patterns observable in mobility data, in this paper, we propose Spaceprint, a fully automated algorithm for finding the repetitive pattern of similar situations in spaces. We evaluate this technique by showing how the latent variables describing the category, and the actual identity of a space can be discovered from the extracted situation patterns. Doing so, we use different real-world mobility datasets with data about the presence of mobile entities in a variety of spaces. We also evaluate the performance of this technique by showing its robustness against uncertainties.

==> implementation.tex <==
\section{Implementation}

There are two parameters that need to be defined in creating a fingerprint; (i) 
Fingerprintsize (ii) minimum resolution. The first parameter is essential in 
defining the fingerprint and there is only one fingerprint duration where the 
fignerprint of the space is meaningful. The second one, however, increases the 

detail level of the fingerprint.
We propose the following method to extract the finger print duration. ...


\begin{algorithm}
   \KwData{$D_n$}
   \KwResult{$Duration$,$Resolution$ }
     \For {$i \leq n$}
       {
          $f_i=Fingerprint(vectorize(D_n,i), 1)$;	\\
       }
       $Duration$= $i$ where $Distance(f_i)$ is minimum;\\
       \For {$i \leq n$}
       {
       	$f_i=Fingerprint(vectorize(D_n,i), 1)$;	\\
       }
       $Resolution$= $i$ where $Distance(f_i)$ is maximum;
       
    \caption{FingerPrintSize}
\end{algorithm}

\subsection{Featurespace}

The important problem here is defining suitable features for fingerprinting the 
space.
Some possible features are, having an opening or 
closing hour, peak hours, groups and individuals, etc. Features that can define 
a space are numerous and each space can be defined by 
various temporal feature. Therefore, defining these features intuitively is not 
an option for classifying any type of space.\\

Our hypothesis is that, 
if we 
define a feature set which can  
represent all usage patterns of the space, we can use it for creating a 
fingerprint. We define such patterns as \textbf{any type of 
synchronous 
presence of groups of probers in the specific period of time}.

We assume that the patterns can be defined in terms of the synchronous presence 
and absence of probers in a certain place. 
To this end, we are interested in $c(t,d,k,T_s)$ which represents 
\textbf{the number of devices} $c$ that were 
present during a \textbf{measurement interval} , 
starting at \textbf{starting time} $t$ and lasting for \textbf{duration} $d$ 
time units, such that the probes are sampled with the frequency of $f_s$ and 
each device had an 
\textbf{absence value} of at least $k$ 
times
during that interval. All of the parameters $t,d,k$ are variables and can have 
all possible values. \\


\begin{tabular}{c|c}\toprule[1.5pt]
\bf Variable Name & \bf Range \\\midrule
$t$  &  ${1 ... W_D}$ \\
$d$ &  ${1 ... (W_D-t)}$ \\
$k$  &  ${0,1}$ \\
$T_s$  &  $1 ... d$ \\
\bottomrule[1.25pt]
\end {tabular}\\

Bellow we explain how the range of these variables is chosen.  Assume we 
measure detections at a given location for some time $\langle 
T,D \rangle$ and study different possible patterns of presence of probers over 
it. The basis our approach to do so is to sample probes with a certain 
frequency for a specific duration 
window of time and count 
the number of probers which appear together in all samples. Both the 
mentioned \textbf{duration window} ($W_D$) and the sampling \textbf{frequency} 
($f_s$) are 
variable.\\
The duration window can be of any 
 length, as long as it is smaller than $D$ ($D\gg W_D$) and it can also start 
 at 
 any time. In other words this window, is a sliding window which can also 
 expand and shrink. Therefore, it can be represented by its start (\textbf{t}) 
 and 
 its length (\textbf{d}). 
\\
 
 Assume probers send out probe messages at a frequency $f_d$ and period $T_d = 
 1/f_d$. In order to understand when few devices are present together we sample 
 probes using sampling frequency $f_s$ and period  $T_s=1/f_s$
 ($T_s \gg 
 T_d$). Additionally, this period cannot be bigger than the duration window 
 ($d\gg T_s$). \\ 
 We first assume that we use only a single 
 physical 
 scanner $S$. If $k=0$, we are 
measuring 
the continuous presence.\\
 If $k=1$, 
we are essentially interested in knowing when a device \emph{came back}. We 
currently consider only the cases $k=0$ and $k=1$.
\\
\\






\begin{algorithm}
	\KwData{$MAC$, $FDuration$, $Resolution$}
	\KwResult{$v$}
	$v=\emptyset$;\\
	\For {$dw \leq FDuration$}
	{	
		\For {$rw \leq dw$}
		{ 
			$u=MAC_{dw}$;\\	
			$append(v,count(u))$;\\
			$u2=MAC_{rw_{dw/rw}}$;\\
			
			\For{ $(j={dw/rw};0;j--)$  }
			{
				${u2}= intersect({u2},MAC_{rw_j})$;\\
				$append(v,count(u2))$;\\
			}
			
			
		}
		
	}	
	
	return($v$);
	\label{algorithm2}
	\caption{vectorize}
\end{algorithm}







 

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{starbucks10n}
		
	\end{subfigure}
	~ 
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{starbucks60n}
		
	\end{subfigure}
	\caption{Choosing Duration}
	
\end{figure}


\subsection{What distance function to use?}
Using the distance function, we are interested to understand how vectors of the 
feature set 
are different from each other. Each element of the vector represent a value 
from a different duration and interval. It is expected that elements that 
elements acquired by a larger big windows and larger small windows have larger 
values than those which represent shorter big windows and shorted small 
windows. Therefore, it is not possible to simply subtract vectors from one 
another. It is necessary that the distance function which is chosen for this 
purpose, normalizes the value such that the effect of each element if equally 
considered important. 
For our experiments we test the distance function mentioned below. In the 
equation mentioned below $v_i$ and $v_j$ are the normalized vectors:
\begin{itemize}
\item \textbf {Total absolute distance (TAD)} $TAD(v_i,v_j)=|v_i-v_j|$
\item \textbf  {Total percentage distance (TPD)}
	 $TPD(v_i,v_j)=\frac{|v_i-v_j|}{|v_i+v_j|}$
 \item \textbf {Mean absolute distance (MAD)} 
 $MAD(v_i,v_j)=\frac{1}{n}|v_i-v_j|$
 \item \textbf {Mean percentage (MPD)}
 $MD(v_i,v_j)=\frac{1}{n}\frac{|v_i-v_j|}{|v_i+v_j|}$


 
 	
\end{itemize}


\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{resolution10080starbucks5}
		
	\end{subfigure}
	~ 
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{resolution1440starbucks5}
		
	\end{subfigure}
	\caption{Choosing Resolution}
	\label{resolutiongraph}
	
\end{figure}

By increasing the resolution, many of the individual presences appear in the 
vector (e.g one device appearing at one small timestamp and leaving). As the 
resolution goes over the average probe frequency this presences does not appear 
in bigger time frames. By normalizing the vector with a large N (MAD distance) 
the vectors the norm of the vectors and their distance becomes smaller. On the 
other hand in a very coarse grained case, we will have very few large values 
that when normalized their limits approach zero.\\

$lim_{N{\rightarrow}{\infty}} ||v||= 
\frac{1}{n{{\rightarrow}{\infty}}}|v_i-v_j|=0$\\
$lim_{N{\rightarrow}0} ||v||=||lim_{N{\rightarrow}1} v_i -lim_{N{\rightarrow}1} 
v_j||$= $lim_{N{\rightarrow}0}||{{1-1}}||= 0$\\, 


Therefore as you can see in the Figure \ref{resolutiongraph} there is a maxima. 
This apex represents the best resolution. 

==> vectorize.tex <==
\section{vectorize}






==> vectorize2.tex <==
\begin{algorithm}
	\KwData{$\set{\overline{DT}}$, $FD$, $FR$}
	\KwResult{$\vec{V}$}
	$\vec{V}=\emptyset$;\\
	\For {$D = R; D \leq FD; D = D + FR$}
	{	\tcc{iterate over all duration window sizes (expanding)}
    	$W = \langle 1,D \rangle$; \\
		\For {$(R = FR; R \leq D; R = R + FR)$}  
		{ 	\tcc{iterate on resolution}
			$u = [\set{\overline{DT}}[W]]_R$;\\	
			$append(v,count(u))$;\\
            $u2 = ???$
			$u2=PL_{Ts_{Dw/Ts}}$;\\
			
			\For{ $(j = {D/R}; 0; j--)$  }
			{
				\tcc{iterate on start (shrink)}
				${u2}= intersect({u2},PL_{Ts_j})$;\\
				$append(V,count(u2))$;\\
			}	
		}	
	}	
	$normv$=$\frac{V}{max(V)}$;
	
	return($normv$);
	\caption{vectorize}
	\label{algorithm2}
	
\end{algorithm}

